BRISC-V Emulator: A Standalone, Installation-Free, Browser-Based Teaching Tool

Many computer organization and computer architecture classes have recently started adopting the RISC-V architecture as an alternative to proprietary RISC ISAs and architectures. Emulators are a common teaching tool used to introduce students to writing assembly. We present the BRISC-V (Boston University RISC-V) Emulator and teaching tool, a RISC-V emulator inspired by existing RISC and CISC emulators. The emulator is a web-based, pure javascript implementation meant to simplify deployment, as it does not require maintaining support for different operating systems or any installation. Here we present the workings, usage, and extensibility of the BRISC-V emulator.

==> Makefile <==
# Add a list of home-made EPS figures here.
PDFFIGURES=figs/arch_pipeline.pdf figs/arch_icswitch.pdf

.SUFFIXES: .fig .eps .ps .dvi .bbl .bib .tex .pdf

FIGURES=${wildcard *.fig}
EPSFIGFILES=${FIGURES:.fig=.eps}
TEXFILES=*.tex

all: pdf   

force: rmdone all

dvi: paper.dvi

xdvi: paper.dvi
	xdvi paper.dvi

gv: paper.ps
	gv paper.ps

ps: paper.ps 

pdf: paper.pdf

rmdone:
	rm -f done.flag

done.flag:
	touch done.flag

printerrors:
	@echo "*****************************"; \
	echo Overview of typeset warnings: ; \
        echo "****************************"; \
	grep "Underfull" paper.log; \
	grep "Overfull" paper.log; \
	echo ; \
        echo "***************************"; \
	echo Overview of latex warnings: ; \
        echo "***************************"; \
	grep "LaTeX Warning" paper.log; \
        echo "***************************"; \
	echo ; \
        echo "***************************"; \
	echo Overview of bibtex warnings: ; \
        echo "***************************"; \
        grep ^Warning-- paper.blg; \
	echo "***************************"; \
	echo ; \
        echo "*************************"; \
	echo Overview of latex errors: ; \
        echo "*************************"; \
	grep "^!" paper.log; \
        echo "*************************"; \
	echo

paper.bbl: paper.bib $(TEXFILES) Makefile done.flag
	pdflatex -interaction=batchmode paper.tex || true
	rm -f $*.pdf
	bibtex -terse $*

paper.pdf: $(TEXFILES) $(PDFFIGFILES) paper.bbl Makefile done.flag
	@echo Running latex once.; \
	while ( pdflatex -interaction=nonstopmode paper.tex; grep Rerun paper.log ) ; do \
          echo; \
          echo "*********************************"; \
          echo "*********************************"; \
          echo Reruning to complete compilation.; \
          echo "*********************************"; \
          echo "*********************************"; \
	done; \
        echo "***************************"; \
	echo DVI file generated.; \
        echo "***************************"; \
	echo ; \
	make printerrors 
			
clean:
	rm -f *.lof *.lot *.pfg *~ *.aux *.dvi *.blg *.log *.bbl $(EPSFIGFILES) *.bak paper.ps paper.pdf *.toc *.swp done.flag




==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios
		Code prettying (Michael D. Adams)
		Two-column formats now balance the last page (ACM request)
		
